Data Unfolding with Wiener-SVD Method

Data unfolding is a common analysis technique used in HEP data analysis. Inspired by the deconvolution technique in the digital signal processing, a new unfolding technique based on the SVD technique and the well-known Wiener filter is introduced. The Wiener-SVD unfolding approach achieves the unfolding by maximizing the signal to noise ratios in the effective frequency domain given expectations of signal and noise and is free from regularization parameter. Through a couple examples, the pros and cons of the Wiener-SVD approach as well as the nature of the unfolded results are discussed.

==> Makefile <==
##########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex 
#main file
texfile = unfolding
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

export TEXINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BSTINPUTS)
#export BIBINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}
	#@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}


==> meta.tex <==

{\LARGE  \textbf META}

Please follow these paper guidelines:
\begin{itemize}
\item Avoid long, convoluted sentences.  \textbf{Brief is beautiful}.
\item Avoid long lines to help git resolve conflicts.
\item Use \textbf{passive voice} (``the thing did something'') not active (\sout{``we saw the thing''})
\item Use the \textbf{siunitx} package for all numbers especially if they have units.  Abbreviations are in the units.tex file.  Feel free to add more.  There are settings of siunitx that can globally change the way its quantities are displayed.  Check these before trying to force something.  Some examples:
  \begin{itemize}
  \item just numbers: ``There were \num{123456} ducks.''  
  \item just units: ``The Fourier transform gives a spectrum in \si{\Hz}''
  \item numbers with units: ``\SI{9.8}{\meter/\second^2}'' or ``\SI{9.8}{\meter\per\second^2}''
  \item you can do ranges: ``\SIrange{-8}{15}{\us}'' and lists ``\SIlist{0.5;1.0;2.0;3.0}{\us}''
  \item units work inside math environment ``$m_{ath} = \SI{6.9}{\GeV}$''  and you can put most common math stuff inside the siunitx macros: ``\num{\sim42}''.
    \item if typing \verb|5\%| is just to short and you want to type more you can do: \verb|\SI{5}{\percent}| giving \SI{5}{\percent}
      
  \end{itemize}
\item Use ``\verb|Figure~\ref{fig:xxx}|'' if it is the subject of the sentence (``Figure 1 shows...'') 
\item Use ``\verb|Fig.~\ref{fig::xxx}|'' if it is the object of the sentence (``The thing is shown in Fig. 2'')
\item Make figure in native \textbf{vector PDF} when possible.
\item Assume paper will be printed in gray scale.  Color is okay but also differentiate plots with different line styles (solid, dashed, etc).
\item It is best to commit all figure making code to the paper repository and the needed input data as \textbf{minimal data files}, such as text files with columns of numbers, JSON, etc.  \textbf{DO NOT} commit large data files.  There's no hard limit but think twice if the file is bigger than 1 MB.
\end{itemize}

Note: comment out this page in the main tex file before sending out drafts.
\pagebreak


==> program.tex <==
\section{Wiener SVD Unfolding Program}\label{sec:program}

The actual computer program based on ROOT .


==> units.tex <==
% This holds some short-hand definitions of macros based on siunitx to
% help keep consistency of quantities and units.

% see
%  http://ctan.org/pkg/siunitx
%  http://mirrors.ctan.org/macros/latex/contrib/siunitx/siunitx.pdf

% Examples:
%  % angles
%  \ang{1.5} off-axis
%
%  % just a unit
%  \si{\kilo\tonne}
%
%  % with a value:
%  \SI{10}{\mega\electronvolt}
%
%  % range of values:
%  \SIrange{60}{120}{\GeV}
%
%  % some number, let LaTeX deal with commas, etc
%  \num{32600}

\usepackage{siunitx}

% some shorthand notation
\DeclareSIUnit \mm {\milli\meter}
\DeclareSIUnit \cm {\centi\meter}
\DeclareSIUnit \us {\micro\second}
\DeclareSIUnit \ms {\milli\second}
\DeclareSIUnit \pA {\pico\ampere}
\DeclareSIUnit \pC {\pico\coulomb}
\DeclareSIUnit \fC {\femto\coulomb}
\DeclareSIUnit \fF {\femto\farrad}
\DeclareSIUnit \pF {\pico\farrad}
\DeclareSIUnit \mV {\milli\volt}
\DeclareSIUnit \kV {\kilo\volt}
\DeclareSIUnit \V {\volt}
\DeclareSIUnit \GOhm {\giga\ohm}
\DeclareSIUnit \MOhm {\mega\ohm}
\DeclareSIUnit \ton {\tonne}
\DeclareSIUnit \kton {\kilo\tonne}
\DeclareSIUnit \kt {\kilo\tonne}
\DeclareSIUnit \Mt {\mega\tonne}
\DeclareSIUnit \eV {\electronvolt}
\DeclareSIUnit \keV {\kilo\electronvolt}
\DeclareSIUnit \MeV {\mega\electronvolt}
\DeclareSIUnit \GeV {\giga\electronvolt}
\DeclareSIUnit \km {\kilo\meter}
\DeclareSIUnit \kW {\kilo\watt}
\DeclareSIUnit \MW {\mega\watt}
\DeclareSIUnit \MHz {\mega\hertz}
\DeclareSIUnit \kHz {\kilo\hertz}
\DeclareSIUnit \mrad {\milli\radian}
\DeclareSIUnit \year {year}
\DeclareSIUnit \POT {POT}
\DeclareSIUnit \sig {$\sigma$}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\lightyear{ly}
\DeclareSIUnit\foot{ft}
\DeclareSIUnit\ft{ft}
% for a bare kt-year
\def\ktyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\year}\xspace}
\def\Mtyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\Mt\year}\xspace}
\def\msr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\meter\steradian}\xspace}
\def\ktMWyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\MW\year}\xspace}

\newcommand{\SIadj}[2]{\SI[number-unit-product = -]{#1}{#2}}
% Adjective form of some common units
% "the 10-kt detector"
\newcommand{\ktadj}[1]{\SIadj{#1}{\kt}}
% "the 1,300-km baseline"
\newcommand{\kmadj}[1]{\SIadj{#1}{\km}}
% "a 567-keV endpoint"
\newcommand{\keVadj}[1]{\SIadj{#1}{\keV}}
% "Typical 20-MeV event"
\newcommand{\MeVadj}[1]{\SIadj{#1}{\MeV}}
% "Typical 2-GeV event"
\newcommand{\GeVadj}[1]{\SIadj{#1}{\GeV}}
% "the 1.2-MW beam"
\newcommand{\MWadj}[1]{\SIadj{#1}{\MW}}
% "the 700-kW beam"
\newcommand{\kWadj}[1]{\SIadj{#1}{\kW}}
% "the 100-tonne beam"
\newcommand{\tonneadj}[1]{\SIadj{#1}{\tonne}}
% "the 4,850-foot depth beam"
\newcommand{\ftadj}[1]{\SIadj{#1}{\ft}}
%

% Mass exposure, people like to put dots between the units
% \newcommand{\ktyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\year}}
% must make usage of \ktyr above consistent with this one before turning on

% Beam x mass exposure, people like to put dots between the units
\newcommand{\ktmwyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\MW\year}}


